SoK: Chasing Accuracy and Privacy, and Catching Both in Differentially Private Histogram Publication

Histograms and synthetic data are of key importance in data analysis. However, researchers have shown that even aggregated data such as histograms, containing no obvious sensitive attributes, can result in privacy leakage. To enable data analysis, a strong notion of privacy is required to avoid risking unintended privacy violations. Such a strong notion of privacy is differential privacy, a statistical notion of privacy that makes privacy leakage quantifiable. The caveat regarding differential privacy is that while it has strong guarantees for privacy, privacy comes at a cost of accuracy. Despite this trade off being a central and important issue in the adoption of differential privacy, there exists a gap in the literature regarding providing an understanding of the trade off and how to address it appropriately. Through a systematic literature review (SLR), we investigate the state-of-the-art within accuracy improving differentially private algorithms for histogram and synthetic data publishing. Our contribution is two-fold: 1) we identify trends and connections in the contributions to the field of differential privacy for histograms and synthetic data and 2) we provide an understanding of the privacy/accuracy trade off challenge by crystallizing different dimensions to accuracy improvement. Accordingly, we position and visualize the ideas in relation to each other and external work, and deconstruct each algorithm to examine the building blocks separately with the aim of pinpointing which dimension of accuracy improvement each technique/approach is targeting. Hence, this systematization of knowledge (SoK) provides an understanding of in which dimensions and how accuracy improvement can be pursued without sacrificing privacy.

==> figures/algorithm-table.tex <==
\begin{table}[htbp]
\centering
\begin{tabularx}{\linewidth}{XrX}          
\textbf{Category} & \textbf{Technique} & \textbf{Algorithm}\\
\rowcolor{gray!10}& Check-then-release & DSAT, DSFT, GGA \\
\rowcolor{gray!10}{\multirow{-2}{*}{Budget Utilization}}& Weighted & BPM \\
 & Error Optimization & AHP, C$i$TM \\
& V-optimal Histogram & NF, SF, P-HP, AHP, DPCube, IHP, mIHP \\
{\multirow{-3}{*}{Clustering}}& Utility Function & EFPA, Outlier-HistoPub \\
\rowcolor{gray!10}& Dependencies & PriSH\\
\rowcolor{gray!10}&  Least Square Minimization & Boost, PMost, BMax, RCF\\
% & &  Linear Program & FPA \\
\rowcolor{gray!10} & Linear Regression & ($\theta$,$\Omega$)-Histogram, $\theta$-CumHisto\\ 
\rowcolor{gray!10}  & Maximum Likelihood & ADMM \\
\rowcolor{gray!10}  & Realizability & C$i$TM\\
\rowcolor{gray!10} {\multirow{-6}{*}{Constrained Inference}} & Sorting & SORTaki \\
 & Bisection & P-HP, Min, Opt IHP, mIHP \\
 & Kd-tree & DPCube \\
{\multirow{-3}{*}{Hierarchical Decomposition}}  & Quadtree & PrivTree\\
\rowcolor{gray!10}{\multirow{1}{*}{Neighbor Relation}}  & Redefine & C$i$TM \\
 &  Data Recycling & RCF\\
{\multirow{-2}{*}{Passive Publishing}}&  Retroactive Grouping & RG\\
\rowcolor{gray!10}& Edge Addition & ($\theta$,$\Omega$)-Histogram, $\theta$-CumHisto \\
\rowcolor{gray!10} & Edge Deletion & T$^\lambda$\\
\rowcolor{gray!10} &  Hashing & PeGS\\
\rowcolor{gray!10}{\multirow{-4}{*}{Projection}}  &  Random Projection & DPPro\\
{\multirow{1}{*}{Sampling}} &  Bernoulli Sampling & RG\\
\rowcolor{gray!10}& Adaptive & DSAT, GGA \\
\rowcolor{gray!10} & Fixed & DSFT \\
\rowcolor{gray!10} &  Truncation & Tru \\
\rowcolor{gray!10}{\multirow{-4}{*}{Threshold}}  &  Wavelet Thresholding & Privelet$^{+}$, Privelet$^{*}$ \\
{\multirow{4}{*}{Transformation}} & Bayesian Network & PrivBayes \\
& Copula Functions & DPCopula \\
 & Fourier Transform & EFPA\\
 &  Wavelet Transform & Privelet\\
\end{tabularx}
\caption{Categorization of techniques used by the different algorithms to achieve accuracy improvement}
\label{table:algorithms}%
\end{table}

%Pythia post-processes by projecting the constraints to get a smaller error. Not sure where it fits?!

==> figures/paper-dimensions-table.tex <==
\begin{table}[htb]
    \centering
    \begin{tabular}{p{0.15\textwidth}|p{0.1\textwidth}p{0.15\textwidth}}
\textbf{Optimization Goal} & \textbf{Addressed Query Size} & \textbf{Algorithm Category} \\
\cellcolor{gray!10}Accumulated Noise& \cellcolor{gray!10}Single &
\cellcolor{gray!10}\begin{tabularx}{0.15\textwidth}{X}
Clustering \\
Transformation 
\end{tabularx}\\
\cellcolor{gray!10}& \cellcolor{white}Workload & \begin{tabularx}{0.15\textwidth}{X}
Budget Utilization \\
\cellcolor{white}Constrained Inference \\
Hierarchical Decomposition\\
\cellcolor{white}Passive Publishing \\
Transformation \\
\cellcolor{white}Threshold
\end{tabularx}\\
Data dimensionality & \cellcolor{gray!10}Workload &
\cellcolor{gray!10}\begin{tabular}{l}
\cellcolor{gray!10}Constrained Inference \\
Projection \\
\cellcolor{gray!10}Transformation\end{tabular} \\
\cellcolor{gray!10}Sensitivity & \cellcolor{white}Single &\begin{tabular}{l}
\cellcolor{white}Clustering \\
Constrained Inference  \\
\cellcolor{white}Projection
\end{tabular} \\ 
\cellcolor{gray!10}& \cellcolor{gray!10}Workload & \cellcolor{gray!10}\begin{tabular}{l}
    Threshold
\end{tabular} \\
\end{tabular}
% \begin{tabular}{p{0.15\textwidth}|p{0.1\textwidth}p{0.15\textwidth}}
% \textbf{Optimization Goal} & \textbf{Addressed Query Size} & \textbf{Algorithm Category} \\ \hline
% {\multirow{8}{*}{Accumulated Noise}}& {\multirow{2}{*}{Single}} & Clustering \\
% & & Transformation \\
% \cline{2-3}
% & {\multirow{4}{*}{Workload}} & Budget Utilization \\
% & & Constrained Inference \\
% & & Hierarchical Decomposition\\
% & & Passive Publishing \\
% & & Transformation \\
% & & Threshold \\
% \hline
% {\multirow{3}{*}{Data dimensionality}}& {\multirow{3}{*}{Workload}} & Constrained Inference \\
% & & Projection \\
% & & Transformation \\
% \hline
% {\multirow{4}{*}{Sensitivity}}
% & {\multirow{3}{*}{Single}} 
%     & Clustering \\
% & & Constrained Inference  \\
% & & Projection\\
% \cline{2-3}
% & {\multirow{1}{*}{Workload}} & Threshold \\
% \hline
% \end{tabular}
 \caption{Different dimensions of accuracy improvement techniques, grouped by the different noise reduction goals}
    \label{table:paper_dimensions}
\end{table}
